Gemini: Integrating Full-fledged Sensing upon Millimeter Wave Communications

Integrating millimeter wave (mmWave)technology in both communication and sensing is promising as it enables the reuse of existing spectrum and infrastructure without draining resources. Most existing systems piggyback sensing onto conventional communication modes without fully exploiting the potential of integrated sensing and communication (ISAC) in mmWave radios (not full-fledged). In this paper, we design and implement a full-fledged mmWave ISAC system Gemini; it delivers raw channel states to serve a broad category of sensing applications. We first propose the mmWave self-interference cancellation approach to extract the weak reflected signals for near-field sensing purposes. Then, we develop a joint optimization scheduling framework that can be utilized in accurate radar sensing while maximizing the communication throughput. Finally, we design a united fusion sensing algorithm to offer a better sensing performance via combining monostatic and bistatic modes. We evaluate our system in extensive experiments to demonstrate Gemini's capability of simultaneously operating sensing and communication, enabling mmWave ISAC to perform better than the commercial off-the-shelf mmWave radar for 5G cellular networks.

==> abstract.tex <==
\begin{abstract}
%Since millimeter wave (mmWave) technology has made substantial advancements in both communication and sensing, a few recent research works have tried to integrate them into the same hardware and spectrum resources. However, their works only consider communication-oriented sensing~(e.g., bistatic sensing mode) and cannot fully explore all potential of integrated sensing and communication~(ISAC) for mmWave.  
%In this paper, we design and implement a revolutionary mmWave ISAC system, \name to bridge the gap between state-of-the-art communication architecture and the new ISAC one. We first propose the mmWave self-interference isolation approach to extract the weak reflected signals for near-field sensing purposes. 
% and then employ an off-the-shelf 60\!~GHz mmWave radio front-ends with 40-element phased arrays to further improve those signals. 
%Then, we develop a joint optimization scheduling framework that can be utilized in accurate radar sensing while maximizing the communication throughput. Finally, we design a united fusion sensing algorithm to offer a better sensing performance via combining monostatic and bistatic modes. We evaluate our system in extensive experiments to demonstrate \name's capability of simultaneously operating sensing and communication, which enables mmWave ISAC to achieve better performance than the commercial off-the-shelf mmWave radar for 5G cellular networks beyond.

\newrev{Since millimeter wave (mmWave) technology has made substantial advancements in both communication and sensing, a few recent research works have tried to integrate them into the same hardware and spectrum resources. However, their works only consider communication-oriented sensing~(e.g., bistatic sensing mode) and cannot fully explore all potential of integrated sensing and communication~(ISAC) for mmWave.  }
In this paper, we design and implement a fully integrated mmWave ISAC system, \name, to bridge the gap between state-of-the-art communication architecture and the new ISAC one. We first propose the mmWave self-interference isolation approach to extract the weak reflected signals for near-field sensing purposes. 
% and then employ an off-the-shelf 60\!~GHz mmWave radio front-ends with 40-element phased arrays to further improve those signals. 
Then, we develop a joint optimization scheduling framework that can be utilized in accurate radar sensing while maximizing the communication throughput. Finally, we design a united fusion sensing algorithm to offer a better sensing performance via combining monostatic and bistatic modes. We evaluate our system in extensive experiments to demonstrate \name's capability of simultaneously operating sensing and communication, which enables mmWave ISAC to achieve better performance than the commercial off-the-shelf mmWave radar for 5G cellular networks beyond.
\end{abstract} 
